Provider Fairness and Beyond-Accuracy Trade-offs in Recommender Systems

Recommender systems, while transformative in online user experiences, have raised concerns over potential provider-side fairness issues. These systems may inadvertently favor popular items, thereby marginalizing less popular ones and compromising provider fairness. While previous research has recognized provider-side fairness issues, the investigation into how these biases affect beyond-accuracy aspects of recommendation systems - such as diversity, novelty, coverage, and serendipity - has been less emphasized. In this paper, we address this gap by introducing a simple yet effective post-processing re-ranking model that prioritizes provider fairness, while simultaneously maintaining user relevance and recommendation quality. We then conduct an in-depth evaluation of the model's impact on various aspects of recommendation quality across multiple datasets. Specifically, we apply the post-processing algorithm to four distinct recommendation models across four varied domain datasets, assessing the improvement in each metric, encompassing both accuracy and beyond-accuracy aspects. This comprehensive analysis allows us to gauge the effectiveness of our approach in mitigating provider biases. Our findings underscore the effectiveness of the adopted method in improving provider fairness and recommendation quality. They also provide valuable insights into the trade-offs involved in achieving fairness in recommender systems, contributing to a more nuanced understanding of this complex issue.

==> sections/02-relatedwork.tex <==
% \ehsan{We can go straight into the litreture review, there is no need for any background here. We can start from section 2.1} \saeedeh{I have removed a single paragraph}
%As recommendation technology advances, researchers are increasingly focused on evaluating the performance of recommender systems, placing a particular emphasis on fairness metrics \cite{deldjoofairness,wang2023survey,li2021tutorial}. This is because fairness is considered a crucial factor in the successful implementation of these systems \cite{amigo2023unifying,mansoury2022understanding}. Due to their reliance on data, recommender systems are vulnerable to bias, which can lead to issues of unfairness and ultimately impact model performance. As such, it is of paramount importance to address and resolve any unfairness issues to ensure the effectiveness of recommender systems. In recommender systems, bias can occur in data, models, and algorithms.In this research, algorithmic bias has been investigated.

Recommender systems play a crucial role in aiding users with important decisions such as medical, financial, and career-related recommendations. However, the presence of bias and unfair recommendations within these systems can have significant and lasting consequences. Minority groups are particularly vulnerable to the negative impacts of such bias, which can greatly harm their lives \cite{deldjoo2021flexible}. Biases may arise on either the item or user side, leading to decreased system efficiency. In this research, we specifically investigate the problem of bias on the item side and will delve into this issue in greater detail.
% \ehsan{maybe add an additional subsection regarding beyond-accuracy metrics so we have  a 2.2, or just remove subsections and make the whole thing just one related work section}
 % \subsection{Algorithmic Item Bias}
 Currently, the most extensively researched form of algorithmic recommendation bias is the popularity bias. This bias is characterized by the tendency for more popular items to be recommended more frequently to certain groups or to all users, as compared to less popular items \cite{abdollahpouri2019unfairness}.
 In recommender systems, items are divided into popular (short-head) and unpopular (long-tail) categories, in the recommendations that are given to users, popular items are more visible even though most of the items are among the unpopular group. Because most of the data is related to these items and in this way, they affect the model, and the group of unpopular items is ignored. This issue causes the problem of popularity bias. In many studies that have been conducted in the field of recommender systems, the popularity bias has been investigated and reduced \cite{abdollah2019managing,naghiaei2022}. Although popular items are likely to match users' preferences and their recommendations contribute to predictive accuracy, users do not consider them to be very useful recommendations because aware of them elsewhere. To measure how well a recommender can expand a user's view of items, a method of presenting less popular items to users is usually introduced \cite{ziegler2005,dong2021user}.
 
 The simplest approach to improve fairness on the item side is to first create a relatively large recommendation list with a classical model and then re-rank the recommendation list. Abdollahpouri et al.~\cite{abdol2019popularity} re-ranked the generated recommendation list by considering the popularity of the item, and Christoffel et al.~\cite{christoffel2015} simply scored each item's recommendation based on its popularity with an adjustable shoulder indicator shared that it greatly reduces the initial points of high recommendations of popular items and thus increases the priority of undesirable items in the recommendation lists. Dong et al.~\cite{dong2019} proposed to linearly collect the ranking numbers of the row and column of the recommendation score matrix obtained by some algorithms in the final recommendation ranking number, where the row and column of the matrix respectively match the user and item. Mansouri et al.~\cite{mansoury2020fair} introduced a general graph-based algorithm for fair improvement of item recommendations. This algorithm repeatedly finds items that are rarely recommended and at the same time are of high quality and adds them to the list of final recommendations of users. Ge et al.~\cite{patro2020} investigated the problem of long-term exposure of items in changing groups with different levels of popularity. They proposed a fairness-constrained reinforcement learning algorithm based on a constrained Markov decision process (CMDP) so that the model can dynamically adjust its recommendation policy.
 


==> sections/XX-outdated.tex <==
% \subsection{Limitations}
% \ehsan{limitations should go to section 6}\saeedeh{changed}
% While existing research on bias has typically focused on accuracy, with an evaluation conducted using well-known metrics like Root Mean Square Error (RMSE) and Normalized Discounter Cumulative Gain (NDCG), recent studies have taken a more comprehensive approach, looking beyond accuracy to metrics such as diversity, novelty, and serendipity. In line with this trend, we have also sought to examine bias in algorithms by utilizing a range of ``beyond-accuracy'' measurements, with a particular focus on provider-side fairness. By adopting a broader set of metrics to evaluate recommender systems, we hope to gain a more nuanced understanding of how these systems function and how they can be improved to ensure fair outcomes for all users.

% Therefore, our main task is to investigate the beyond-accuracy metric with respect to provider-side fairness and bias. By examining additional criteria such as novelty, diversity, and serendipity, we can better understand how to create a more equitable production process. Our focus is on ensuring that all parties involved have an equal opportunity to participate and succeed, free from discrimination and bias. Through this investigation, we can identify best practices for providers to adopt, promoting a more just and fair environment for all.

